VidCompress: Memory-Enhanced Temporal Compression for Video Understanding in Large Language Models

Video-based multimodal large language models (Video-LLMs) possess significant potential for video understanding tasks. However, most Video-LLMs treat videos as a sequential set of individual frames, which results in insufficient temporal-spatial interaction that hinders fine-grained comprehension and difficulty in processing longer videos due to limited visual token capacity. To address these challenges, we propose VidCompress, a novel Video-LLM featuring memory-enhanced temporal compression. VidCompress employs a dual-compressor approach: a memory-enhanced compressor captures both short-term and long-term temporal relationships in videos and compresses the visual tokens using a multiscale transformer with a memory-cache mechanism, while a text-perceived compressor generates condensed visual tokens by utilizing Q-Former and integrating temporal contexts into query embeddings with cross attention. Experiments on several VideoQA datasets and comprehensive benchmarks demonstrate that VidCompress efficiently models complex temporal-spatial relations and significantly outperforms existing Video-LLMs.

==> tabs/ablation_memvit.tex <==
% Table generated by Excel2LaTeX from sheet 'ablation'
\begin{table}[!t]
  \centering
  \caption{Add caption}
    \begin{tabular}{c|ccccc}
    \toprule
    \multirow{2}[2]{*}{Model Type} & \multicolumn{4}{c}{Video-MME} & \multirow{2}[2]{*}{MVB} \\
          & short & medium & long  & all   &  \\
    \midrule
    wo memvit & 44.3  & 38.6  & 37.3  & 40.7  & 43.4  \\
    ours  & 46.4  & 41.9  & 37.8  & 43.0  & 46.9  \\
    \midrule
    $\Delta$ & +2.1  & +3.3  & +0.5  & +2.3  & +3.5 \\
    \bottomrule
    \end{tabular}%
  \label{tab:ab_memvit}%
\end{table}%

